Classifier-Free Guidance: From High-Dimensional Analysis to Generalized Guidance Forms

Classifier-Free Guidance (CFG) is a widely adopted technique in diffusion and flow-based generative models, enabling high-quality conditional generation. A key theoretical challenge is characterizing the distribution induced by CFG, particularly in high-dimensional settings relevant to real-world data. Previous works have shown that CFG modifies the target distribution, steering it towards a distribution sharper than the target one, more shifted towards the boundary of the class. In this work, we provide a high-dimensional analysis of CFG, showing that these distortions vanish as the data dimension grows. We present a blessing-of-dimensionality result demonstrating that in sufficiently high and infinite dimensions, CFG accurately reproduces the target distribution. Using our high-dimensional theory, we show that there is a large family of guidances enjoying this property, in particular non-linear CFG generalizations. We study a simple non-linear power-law version, for which we demonstrate improved robustness, sample fidelity and diversity. Our findings are validated with experiments on class-conditional and text-to-image generation using state-of-the-art diffusion and flow-matching models.

==> z_additional_plots.tex <==
\clearpage

\subsubsection[Qualitative analysis: fixed non-linear parameter]{Qualitative analysis: varying $\omega$, fixed $\alpha$.}
\label{sec:qualit_anal_fix_alpha}

\ifarxiv
    \begin{figure}[h]
        \centering
        \begin{subfigure}[t]{0.48\textwidth} % Adjust width to fit two columns
            \centering
            \includegraphics[width=\linewidth]{assets/plots/changing_omega-1.pdf}
            \caption{Class \textit{107: jellyfish} with $\alpha=0.$}
        \end{subfigure}%
        \hfill
        \begin{subfigure}[t]{0.48\textwidth} % Adjust width to fit two columns
            \centering
            \includegraphics[width=\linewidth]{assets/plots/changing_omega-2.pdf}
            \caption{Class \textit{107: jellyfish} with $\alpha=0.9$}
        \end{subfigure}
        \vspace{0.3cm} % Adjust vertical space
        \begin{subfigure}[t]{0.48\textwidth} % Adjust width to fit two columns
            \centering
            \includegraphics[width=\linewidth]{assets/plots/changing_omega-5.pdf}
            \caption{Class \textit{309: bee} with $\alpha=0.$}
        \end{subfigure}%
        \hfill
        \begin{subfigure}[t]{0.48\textwidth} % Adjust width to fit two columns
            \centering
            \includegraphics[width=\linewidth]{assets/plots/changing_omega-6.pdf}
            \caption{Class \textit{309: bee} with $\alpha=0.9$}
        \end{subfigure}
        \vspace{0.3cm} % Adjust vertical space
        \begin{subfigure}[t]{0.48\textwidth} % Adjust width to fit two columns
            \centering
            \includegraphics[width=\linewidth]{assets/plots/changing_omega-3.pdf}
            \caption{Class \textit{305: dung beetle} with $\alpha=0.$}
        \end{subfigure}%
        \hfill
        \begin{subfigure}[t]{0.48\textwidth} % Adjust width to fit two columns
            \centering
            \includegraphics[width=\linewidth]{assets/plots/changing_omega-4.pdf}
            \caption{Class \textit{305: dung beetle} with $\alpha=0.9$}
        \end{subfigure}
        \caption{Generated images for different classes with varying values of $\omega$ and $\alpha$. Each panel shows the effect of changing $\alpha$ from 0 to 0.9, demonstrating the impact on diversity and image quality.}
    \end{figure}
\else
    \begin{figure}[h]
        \centering
        \subfigure[Class \textit{107: jellyfish} with $\alpha=0.$]{
            \includegraphics[width=0.48\textwidth]{assets/plots/changing_omega-1.pdf}
        }%
        \hfill
        \subfigure[Class \textit{107: jellyfish} with $\alpha=0.9$]{
            \includegraphics[width=0.48\textwidth]{assets/plots/changing_omega-2.pdf}
        }
        \vspace{0.3cm} % Adjust vertical space
        \subfigure[Class \textit{309: bee} with $\alpha=0.$]{
            \includegraphics[width=0.48\textwidth]{assets/plots/changing_omega-5.pdf}
        }%
        \hfill
        \subfigure[Class \textit{309: bee} with $\alpha=0.9$]{
            \includegraphics[width=0.48\textwidth]{assets/plots/changing_omega-6.pdf}
        }
        \vspace{0.3cm} % Adjust vertical space
        \subfigure[Class \textit{305: dung beetle} with $\alpha=0.$]{
            \includegraphics[width=0.48\textwidth]{assets/plots/changing_omega-3.pdf}
        }%
        \hfill
        \subfigure[Class \textit{305: dung beetle} with $\alpha=0.9$]{
            \includegraphics[width=0.48\textwidth]{assets/plots/changing_omega-4.pdf}
        }
        \caption{Generated images for different classes for varying values of $\omega$ and $\alpha$. Each panel shows the effect of changing $\alpha$ from 0 to 0.9, demonstrating the impact on diversity and image quality.}
    \end{figure}
\fi

\clearpage

\subsubsection[ualitative analysis: fixed guidance scale]{Qualitative analysis: fixed $\omega$, varying $\alpha$.}
\label{sec:qualit_anal_fix_omega}

\ifarxiv
    \begin{figure}[h]
        \centering
        \begin{subfigure}[t]{0.4\textwidth} % Increase width to 0.48
            \centering
            \includegraphics[width=\linewidth]{assets/plots/changing_alpha-8.pdf}
            \caption{Prompt \textit{bear in its natural habitat}}
        \end{subfigure}%
        \hfill
        \begin{subfigure}[t]{0.4\textwidth} % Increase width to 0.48
            \centering
            \includegraphics[width=\linewidth]{assets/plots/changing_alpha-6.pdf}
            \caption{Prompt \textit{a bouquet of roses}}
        \end{subfigure}
        \vspace{0.3cm} % Reduce vertical space
        \begin{subfigure}[t]{0.4\textwidth} % Increase width to 0.48
            \centering
            \includegraphics[width=\linewidth]{assets/plots/changing_alpha-7.pdf}
            \caption{Prompt \textit{a bowl of citrus fruit}}
        \end{subfigure}%
        \hfill
        \begin{subfigure}[t]{0.4\textwidth} % Increase width to 0.48
            \centering
            \includegraphics[width=\linewidth]{assets/plots/changing_alpha-5.pdf}
            \caption{Prompt \textit{a simple drawing of a smiling sun}}
        \end{subfigure}
        \vspace{-.35cm}
        \caption{T2IM generated images for different prompts with $\omega=4.$ and varying value of $\alpha$.}
        \vspace{-.4cm}
    \end{figure}
    
    \begin{figure}[h]
        \centering
        \begin{subfigure}[t]{0.4\textwidth} % Increase width to 0.48
            \centering
            \includegraphics[width=\linewidth]{assets/plots/changing_alpha-1.pdf}
            \caption{Class \textit{107: jellyfish}}
        \end{subfigure}%
        \hfill
        \begin{subfigure}[t]{0.4\textwidth} % Increase width to 0.48
            \centering
            \includegraphics[width=\linewidth]{assets/plots/changing_alpha-2.pdf}
            \caption{Class \textit{305: dung beetle}}
        \end{subfigure}
        \vspace{0.3cm} % Reduce vertical space
        \begin{subfigure}[t]{0.4\textwidth} % Increase width to 0.48
            \centering
            \includegraphics[width=\linewidth]{assets/plots/changing_alpha-3.pdf}
            \caption{Class \textit{309: bee}}
        \end{subfigure}%
        \hfill
        \begin{subfigure}[t]{0.4\textwidth} % Increase width to 0.48
            \centering
            \includegraphics[width=\linewidth]{assets/plots/changing_alpha-4.pdf}
            \caption{Class \textit{959: carbonara}}
        \end{subfigure}
        \vspace{-.35cm}
        \caption{CC generated images for different classes with $\omega=4.$ and varying value of $\alpha$.}
    \end{figure}
\else
    \begin{figure}[h]
        \centering
        \subfigure[Prompt \textit{bear in its natural habitat}]{
            \includegraphics[width=0.4\textwidth]{assets/plots/changing_alpha-8.pdf}
        }%
        \hfill
        \subfigure[Prompt \textit{a bouquet of roses}]{
            \includegraphics[width=0.4\textwidth]{assets/plots/changing_alpha-6.pdf}
        }
        \vspace{0.3cm} % Reduce vertical space
        \subfigure[Prompt \textit{a bowl of citrus fruit}]{
            \includegraphics[width=0.4\textwidth]{assets/plots/changing_alpha-7.pdf}
        }%
        \hfill
        \subfigure[Prompt \textit{a simple drawing of a smiling sun}]{
            \includegraphics[width=0.4\textwidth]{assets/plots/changing_alpha-5.pdf}
        }
        \vspace{-0.35cm} % Adjust vertical space
        \caption{T2IM generated images for different prompts with $\omega=4.$ and varying value of $\alpha$.}
        \vspace{-0.4cm} % Adjust vertical space
    \end{figure}
    \begin{figure}[h]
        \centering
        \subfigure[Class \textit{107: jellyfish}]{
            \includegraphics[width=0.4\textwidth]{assets/plots/changing_alpha-1.pdf}
        }%
        \hfill
        \subfigure[Class \textit{305: dung beetle}]{
            \includegraphics[width=0.4\textwidth]{assets/plots/changing_alpha-2.pdf}
        }
        \vspace{0.3cm} % Reduce vertical space
        \subfigure[Class \textit{309: bee}]{
            \includegraphics[width=0.4\textwidth]{assets/plots/changing_alpha-3.pdf}
        }%
        \hfill
        \subfigure[Class \textit{959: carbonara}]{
            \includegraphics[width=0.4\textwidth]{assets/plots/changing_alpha-4.pdf}
        }
        \vspace{-0.35cm} % Adjust vertical space
        \caption{CC generated images for different classes with $\omega=4.$ and varying value of $\alpha$.}
    \end{figure}
\fi
